Towards a More Reliable and Available Docker-based Container Cloud

Operating System-level virtualization technology, or containers as they are commonly known, represents the next generation of light-weight virtualization, and is primarily represented by Docker. However, Docker's current design does not complement the SLAs from Docker-based container cloud offerings promising both reliability and high availability. The tight coupling between the containers and the Docker daemon proves fatal for the containers' uptime during daemon's unavailability due to either failure or upgrade. We present the design and implementation of HYDRA, which fundamentally isolates the containers from the running daemon. Our evaluation shows that HYDRA imposes only moderate overheads even under load, while achieving much higher container availability.

==> sections/background.tex <==
\section{\docker}
\label{sec:docker}

\docker\ is one of the fastest growing container technology, and has been 
adopted by leading firms world over, such as Baidu, eBay, PayPal, Yelp, etc. It 
follows a client-server model, where the client is the primary user interface 
for accepting commands, and communicates back and forth with a \docker\ daemon, 
which is responsible for building and running the containers. The \docker\ 
system consists of the following major components:

\begin{mylist}
 \item \textbf{Image} is a basic building block in \docker. Images can be 
configured with applications, and are used as templates to create containers. 
They are organized as layers, with every change added as another layer on the 
top.

 \item \textbf{Registry} is a repository for \docker\ images, and can be either 
public or private. A registry enables easy distribution of images.

 \item \textbf{Container} is an execution environment built from a corresponding 
image. \docker\ provides this light-weight process-level virtualization using 
the Linux Kernel features like (i) namespaces (to isolate process workspace), 
(ii) control groups (to share resources), and (iii) copy-on-write union file 
system (for backend storage).
% It combines these components into a wrapper container format called 
% \textit{libcontainer}, which serves as a template to create containers atop 
% the  OS.
\end{mylist}

% \myparagraph{Design trade-offs} As per the current \docker\ architecture, 
% containers are spawned as direct descendants of the \docker\ daemon (see 
% Figure~\ref{figure:docker}), which performs a \code{wait} \todo{add text.}. 
% While this parent-child relationship provides a straight forward way of 
% signaling/communication, it also critically affects a container's up-time, 
% stability and high availability. Specifically,
% 
% \begin{mylist}
%  \item Daemon's death (due to a restart, kill, or abrupt crash resulting from 
% bug(s) in \docker\ code) aborts all the running containers as well. 
%  \item An upgrade/fix to daemon can not be performed without impacting the 
% up-time/stability of the containers.
% \end{mylist}

% Both these issues become even more important in production environments, like  
% container clouds, where different containers running on a server might belong 
% to same or different clients and might host highly available or stateless 
% services. In such scenarios, a container downtime caused by external factors 
% such as a daemon's death/upgrade, is highly undesirable.

==> sections/design.tex <==
\section{Alternate designs}
\label{sec:alternate}

\subsection{Lazy \tool}
\label{sec:alternate:lazy}

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{figs/architecture.png}
\caption{Lazy \tool\ architecture. \note{This is a place holder.}}
\label{figure:lazy-tool}
\end{figure}

We also considered a \textit{lazy} version of \tool, where newly spawned 
monitors (along with their containers) are initially direct children of the 
\docker\ daemon, as in existing \docker\ implementation. However, upon daemon 
failure (due to abrupt crash or upgrade), all the monitors (along with their 
running containers) become orphan and are adopted by the top-level INIT process. 
Figure~\ref{figure:lazy-tool} presents a schematic architecture of the lazy 
\tool.

When the \docker\ daemon restarts, it detects presence of old executing 
containers and manages them through communication mechanisms described 
in~\xref{sec:tool:design:communication}. Communication with containers in the 
daemon's process hierarchy also utilizes the functionality, \ie\ direct signals 
(for managing container execution state), and external APIs (for managing 
resources and control plane I/O). Note that currently \docker\ also detects such 
containers, but kills them and cleans all state corresponding to them.

%% what are the differences
The lazy implementation of \tool\ as described above has less homogeneity from a 
design perspective, with the containers attached to both the \docker\ daemon and 
the INIT processes. 
% Moreover, this design introduces complexity in the monitor code, since the 
% monitor must now use different mechanisms to communicate with the daemon 
% depending on whether it is an orphan or not. 
However, since both versions of \tool\ require spawning a monitor process per 
container, they result in similar performance. \note{Not sure about this. Fix it 
after the experiments.}

\subsection{runC}
\label{sec:alternate:runC}

runC~\cite{runc} is a CLI tool for spawning and running containers according to 
the Open Container Specification~\cite{oc}. Specifically, containers are spawned 
children of the runC process, and can be embedded into other systems without 
having to run a \docker\ daemon.

%% what are the differences
While runC is similar in spirit to \tool, and decouples the containers from the 
orchestration platform, it does not provide any mechanisms to operate the 
functioning of the several runC containers. Currently, runC is a stand alone 
tool, without any future plans of being adopted by the \docker\ 
community~\cite{proposal}. In contrast, \tool\ is compatible with the current 
\docker\ eco-system.

==> sections/discussion.tex <==
\section{Limitations}
\label{sec:limitations}

==> sections/motivation.tex <==
\section{Motivation}
\label{sec:motivation}

